Fixed $\beta$-VAE Encoding for Curious Exploration in Complex 3D Environments

Curiosity is a general method for augmenting an environment reward with an intrinsic reward, which encourages exploration and is especially useful in sparse reward settings. As curiosity is calculated using next state prediction error, the type of state encoding used has a large impact on performance. Random features and inverse-dynamics features are generally preferred over VAEs based on previous results from Atari and other mostly 2D environments. However, unlike VAEs, they may not encode sufficient information for optimal behaviour, which becomes increasingly important as environments become more complex. In this paper, we use the sparse reward 3D physics environment Animal-AI, to demonstrate how a fixed $\beta$-VAE encoding can be used effectively with curiosity. We combine this with curriculum learning to solve the previously unsolved exploration intensive detour tasks while achieving 22\% gain in sample efficiency on the training curriculum against the next best encoding. We also corroborate the results on Atari Breakout, with our custom encoding outperforming random features and inverse-dynamics features.

==> reference.tex <==
@Article{DeepakCuriosity,
Author = "Pathak, Deepak and Agrawal, Pulkit and Efros, Alexei A and Darrell, Trevor",
Title = "Curiosity-driven Exploration by Self-supervised Prediction",
Journal = "Arxiv",
ArxivId = {1705.05363v1},
year = 2017
}

@Article{CURL,
Author = "Srinivas, Aravind and Laskin, Michael and Abbeel, Pieter",
Title = "CURL: Contrastive Unsupervised Representations for Reinforcement Learning",
Journal = "Arxiv",
year = 2020
}

@Article{CuriosityReview,
Author = "Burda, Yuri and Edwards, Harri and Pathak, Deepak and Storkey, Amos and Darrell, Trevor and Efros, Alexei A",
Title = "Large-Scale Study of Curiosity-Driven Learning",
Journal = "ICLR",
ArxivId = {1808.04355v1},
year = 2019
}

@Misc{CurriculumLearning,
Author = "Lilian Weng",
Title = "Curriculum for Reinforcement Learning",
Note = "https://lilianweng.github.io",
year = 2020
}

@Article{AnimalAI-Testbed,
Author = "Crosby, M. and
Beyret, B. and 
Shanahan, M. and 
Hernández-Orallo, J. and 
Cheke, L. and
Halina, M.",
Title = "The Animal-AI Testbed and Competition",
Journal = "Proceedings of the NeurIPS 2019 Competition and Demonstration Track, in PMLR 123:164-176",
year = 2020
}

@article{shanahan2020artificial,
  title={Artificial intelligence and the common sense of animals},
  author={Shanahan, Murray and Crosby, Matthew and Beyret, Benjamin and Cheke, Lucy},
  journal={Trends in cognitive sciences},
  year={2020},
  publisher={Elsevier}
}


@Article{AnimalAI-Environment,
Author = "Beyret, Benjamin and Hernandez-Orallo, Jose and Cheke, Lucy and Halina, Marta and Shanahan, Murray and Crosby, Matthew",
Title = "The Animal-AI Environment: Training and Testing Animal-Like Artificial Cognition",
year = 2019
}

@Article{PPO,
Author = " Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec
and Oleg, Klimov", 
Title = "Proximal Policy Optimization Algorithms",
year = 2017
}

@article{TRPO,
  author    = {John Schulman and
               Sergey Levine and
               Philipp Moritz and
               Michael I. Jordan and
               Pieter Abbeel},
  title     = {Trust Region Policy Optimization},
  journal   = {CoRR},
  volume    = {abs/1502.05477},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.05477},
  archivePrefix = {arXiv},
  eprint    = {1502.05477},
  timestamp = {Mon, 13 Aug 2018 16:48:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/SchulmanLMJA15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{Bootcamp,
Author = "Deep RL Google Bootcamp ",
Title = "Deep RL Bootcamp Lecture 5",
Note = "https://www.youtube.com/watch?v=xvRrgxcpaHY",
year = 2017
}

@article{vector-state,
  author    = {Yarats, Denis and Zhang, Amy and Kostrikov, Ilya and Amos, Brandon and Pineau, Joelle and Fergus, Rob},
  title     = {Improving Sample Efficiency in Model-Free Reinforcement Learning from Images},
  year = 2019
  }
  
  @article{curriculum-learning,
  author    = {Bengio, Yoshua and
Louradour, Jérôme and
Collobert, Ronan and
Weston, Jason},
  title     = {Curriculum Learning},
  year = 2009
  }

@article{curriculum-difficulty,
  author    = {Justesen, Niels and Torrado,Ruben Rodriguez and
  Bontrager, Philip and Khalifa, Ahmed},
  title     = {Illuminating Generalization in Deep Reinforcement Learning through Procedural Level Generation},
  year = 2018
  }
  
@article{curriculum-forget,
  author    = { Zaremba, Wojciech and Sutskever, Ilya},
  title     = {Learning to Execute},
  year = 2014
  }
  
 @book{sutton1998introduction,
  title={Introduction to reinforcement learning},
  author={Sutton, Richard S and Barto, Andrew G and others},
  volume={135},
  year={1998},
  publisher={MIT press Cambridge}
}

@article{beta-vae,
  author    = { Higgins, Irina and 
Matthey, Loic and 
Pal, Arka and
Burgess, Christopher and 
Glorot, Xavier
},
  title     = {$\beta$-VAE: LEARNING BASIC VISUAL CONCEPTS WITH A
CONSTRAINED VARIATIONAL FRAMEWORK },
  year = 2017
  }
  
@article{unity,
author    = { Juliani, Arthur and 
Berges, Vincent-Pierre
},
title     = {Unity: A general platform for intelligent agents.},
year = 2018
}

@article{sac,
author    = { Haarnoja, Tuomas and Zhou, Aurick
},
title     = {Soft Actor-Critic Algorithms and Applications},
year = 2019
}

@article{psy,
author    = { Ryan, Richard and Deci, Edward
},
title     = {Intrinsic and extrinsic motivations: Classic definitions and new directions.},
year = 2000
}

@article{first,
author    = { Schmidhuber, Jurgen
},
title     = {A possibility for implementing curiosity and boredom in model-building neural controllers..},
year = 1991
}

@article{agent57,
author    = { Badia, Adrià and
Piot, Bilal and 
Kapturowski, Steven and 
Sprechmann, Pablo and 
Vitvitskyi, Alex and 
Guo,Daniel  and 
Blundell, Charles
},
title     = {Agent57: Outperforming the Atari Human Benchmark},
year = 2020
}

@article{real-world,
author    = {
Dulac-Arnold, Gabriel and 
Mankowitz, Daniel and
Hester, Todd
},
title     = {Challenges of Real-World Reinforcement Learning},
year = 2019
}

@article{kingma,
author    = {
Kingma, Diederik and 
Welling, Max 
},
title     = {Auto-Encoding Variational Bayes},
year = 2013
}

@article{curious-robot,
author    = {
Sandy, Huang and
Martina, Zambelli and
Jackie,  Kay
},
title     = {Learning Gentle Object Manipulation with
Curiosity-Driven Deep Reinforcement Learning},
year = 2019
}

@article{2018arXivUMAP,
author = {{McInnes}, L. and {Healy}, J. and {Melville}, J.},
title = "{UMAP: Uniform Manifold Approximation
and Projection for Dimension Reduction}",
journal = {ArXiv e-prints},
archivePrefix = "arXiv",
eprint = {1802.03426},
primaryClass = "stat.ML",
keywords = {Statistics - Machine Learning,
         Computer Science - Computational Geometry,
         Computer Science - Learning},
year = 2018,
month = feb,
}

@misc{burda2018exploration,
      title={Exploration by Random Network Distillation}, 
      author={Yuri Burda and Harrison Edwards and Amos Storkey and Oleg Klimov},
      year={2018},
      eprint={1810.12894},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{anand2020unsupervised,
      title={Unsupervised State Representation Learning in Atari}, 
      author={Ankesh Anand and Evan Racah and Sherjil Ozair and Yoshua Bengio and Marc-Alexandre Côté and R Devon Hjelm},
      year={2020},
      eprint={1906.08226},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{pere2018unsupervised,
      title={Unsupervised Learning of Goal Spaces for Intrinsically Motivated Goal Exploration}, 
      author={Alexandre Péré and Sébastien Forestier and Olivier Sigaud and Pierre-Yves Oudeyer},
      year={2018},
      eprint={1803.00781},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{luo2019curiosity,
  title={Curiosity-driven reinforcement learning for diverse visual paragraph generation},
  author={Luo, Yadan and Huang, Zi and Zhang, Zheng and Wang, Ziwei and Li, Jingjing and Yang, Yang},
  booktitle={Proceedings of the 27th ACM International Conference on Multimedia},
  pages={2341--2350},
  year={2019}
}

@article{zhao2019curiosity,
  title={Curiosity-driven experience prioritization via density estimation},
  author={Zhao, Rui and Tresp, Volker},
  journal={arXiv preprint arXiv:1902.08039},
  year={2019}
}

@article{huang2019learning,
  title={Learning gentle object manipulation with curiosity-driven deep reinforcement learning},
  author={Huang, Sandy H and Zambelli, Martina and Kay, Jackie and Martins, Murilo F and Tassa, Yuval and Pilarski, Patrick M and Hadsell, Raia},
  journal={arXiv preprint arXiv:1903.08542},
  year={2019}
}

@article{juliani2018unity,
  title={Unity: A general platform for intelligent agents},
  author={Juliani, Arthur and Berges, Vincent-Pierre and Teng, Ervin and Cohen, Andrew and Harper, Jonathan and Elion, Chris and Goy, Chris and Gao, Yuan and Henry, Hunter and Mattar, Marwan and others},
  journal={arXiv preprint arXiv:1809.02627},
  year={2018}
}

@article{bellemare2016unifying,
  title={Unifying count-based exploration and intrinsic motivation},
  author={Bellemare, Marc G and Srinivasan, Sriram and Ostrovski, Georg and Schaul, Tom and Saxton, David and Munos, Remi},
  journal={arXiv preprint arXiv:1606.01868},
  year={2016}
}

@article{achiam2017surprise,
  title={Surprise-based intrinsic motivation for deep reinforcement learning},
  author={Achiam, Joshua and Sastry, Shankar},
  journal={arXiv preprint arXiv:1703.01732},
  year={2017}
}

@article{chiandetti2011intuitive,
  title={Intuitive physical reasoning about occluded objects by inexperienced chicks},
  author={Chiandetti, Cinzia and Vallortigara, Giorgio},
  journal={Proceedings of the Royal Society B: Biological Sciences},
  volume={278},
  number={1718},
  pages={2621--2627},
  year={2011},
  publisher={The Royal Society}
}

@article{smith2010well,
  title={How well do dingoes, Canis dingo, perform on the detour task?},
  author={Smith, Bradley Philip and Litchfield, Carla Anita},
  journal={Animal Behaviour},
  volume={80},
  number={1},
  pages={155--162},
  year={2010},
  publisher={Elsevier}
}

@article{maclean2014evolution,
  title={The evolution of self-control},
  author={MacLean, Evan L and Hare, Brian and Nunn, Charles L and Addessi, Elsa and Amici, Federica and Anderson, Rindy C and Aureli, Filippo and Baker, Joseph M and Bania, Amanda E and Barnard, Allison M and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={111},
  number={20},
  pages={E2140--E2148},
  year={2014},
  publisher={National Acad Sciences}
}

@article{lake2017building,
  title={Building machines that learn and think like people},
  author={Lake, Brenden M and Ullman, Tomer D and Tenenbaum, Joshua B and Gershman, Samuel J},
  journal={Behavioral and brain sciences},
  volume={40},
  year={2017},
  publisher={Cambridge University Press}
}

@article{friston2009free,
  title={The free-energy principle: a rough guide to the brain?},
  author={Friston, Karl},
  journal={Trends in cognitive sciences},
  volume={13},
  number={7},
  pages={293--301},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{han2020curiosity,
  title={Curiosity-Driven Variational Autoencoder for Deep Q Network},
  author={Han, Gao-Jie and Zhang, Xiao-Fang and Wang, Hao and Mao, Chen-Guang},
  booktitle={Pacific-Asia Conference on Knowledge Discovery and Data Mining},
  pages={764--775},
  year={2020},
  organization={Springer}
}

 @InProceedings{pmlr-v70-higgins17a, title = {{DARLA}: Improving Zero-Shot Transfer in Reinforcement Learning}, author = {Irina Higgins and Arka Pal and Andrei Rusu and Loic Matthey and Christopher Burgess and Alexander Pritzel and Matthew Botvinick and Charles Blundell and Alexander Lerchner}, booktitle = {Proceedings of the 34th International Conference on Machine Learning}, pages = {1480--1490}, year = {2017}, editor = {Doina Precup and Yee Whye Teh}, volume = {70}, series = {Proceedings of Machine Learning Research}, address = {International Convention Centre, Sydney, Australia}, month = {06--11 Aug}, publisher = {PMLR}, pdf = {http://proceedings.mlr.press/v70/higgins17a/higgins17a.pdf}, url = {http://proceedings.mlr.press/v70/higgins17a.html}, abstract = {Domain adaptation is an important open problem in deep reinforcement learning (RL). In many scenarios of interest data is hard to obtain, so agents may learn a source policy in a setting where data is readily available, with the hope that it generalises well to the target domain. We propose a new multi-stage RL agent, DARLA (DisentAngled Representation Learning Agent), which learns to see before learning to act. DARLA’s vision is based on learning a disentangled representation of the observed environment. Once DARLA can see, it is able to acquire source policies that are robust to many domain shifts – even with no access to the target domain. DARLA significantly outperforms conventional baselines in zero-shot domain adaptation scenarios, an effect that holds across a variety of RL environments (Jaco arm, DeepMind Lab) and base RL algorithms (DQN, A3C and EC).} } 
 
 @article{ha2018world,
  title={World models},
  author={Ha, David and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1803.10122},
  year={2018}
}

@article{beattie2016deepmind,
  title={Deepmind lab},
  author={Beattie, Charles and Leibo, Joel Z and Teplyashin, Denis and Ward, Tom and Wainwright, Marcus and K{\"u}ttler, Heinrich and Lefrancq, Andrew and Green, Simon and Vald{\'e}s, V{\'\i}ctor and Sadik, Amir and others},
  journal={arXiv preprint arXiv:1612.03801},
  year={2016}
}
